From Search Agents to Dissemination Interfaces: Understanding Human Trust in Health Information from Conversational Search

Large Language Models (LLMs) deployed through Conversational User Interfaces (CUIs) are transforming health information-seeking by offering immediate, interactive experiences compared to traditional search engines like Google. However, how trust is influenced by both the types of search agents and the interface used to disseminate the information remains underexplored. This research integrates two mixed-methods studies (lab sessions and interviews) to comprehensively explore trust perceptions in health information across different search agents and dissemination interfaces. In Study 1 (N=21), we investigated trust in health information sourced from ChatGPT and Google across three types of health-related search tasks. Results showed significantly higher trust in health information from ChatGPT, highlighting the promise of LLM-powered conversational search. Building on this, Study 2 (N=20) extended the investigation to explore how the dissemination interface influences trust in LLM-sourced health information by comparing three interfaces: text-based, speech-based, and embodied, all sourcing from the same LLM. Findings revealed significant trust variations across the dissemination interfaces. Interviews from both studies revealed key factors influencing trust in LLM-powered conversational search, including source credibility, participants' search autonomy, and prior knowledge as well as the interaction style and modality. Our findings highlight the potential of LLM-powered conversational search to transform health information-seeking, underscoring the interplay between the credible search agents and the thoughtfully designed dissemination interfaces in shaping trust. These insights are crucial for developing effective, trustworthy LLM-powered health tools to enhance the health information-seeking experience.

==> main/trust-interface/mixlm_result.tex <==

\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.00}
\begin{tabularx}{\columnwidth}{p{6.5cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X
 >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X}
\toprule
\textbf{Scores} & \textbf{Coef. ($\beta$)} & \textbf{Std.Err.} & \textbf{P-value} \\
\hline

Trust in information (Text vs. Embodied) & 0.195 & 0.089 & \textbf{0.029} \\

Trust in information (Text vs. Speech) & 0.012 & 0.072 & 0.865 \\

Trust in information (Speech vs. Embodied) & 0.182 & 0.058 & \textbf{0.002} \\

\hline

Trust in interfaces & 0.195 & 0.120 & 0.106 \\
Usability level & 0.194 & 0.064 & \textbf{0.003} \\
Familiarity level & 0.127 & 0.068 & 0.060 \\

\bottomrule
\end{tabularx}
\caption{
Results from the Mixed Linear Model (MixedLM) analysis. 
The coefficient (``Coef.'') represents the estimated effect size of a predictor variable on the dependent variable (``trust in information'').
% The standard error (``Std.Err.'') measures the precision of the coefficient estimate. 
The P-value represents the significance level of the differences.
}
\vspace{-5mm}
\label{mixedlm}
\end{table}

==> main/trust-search/anova_res.tex <==
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.25}
\begin{tabularx}{\columnwidth}{p{4cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X
 >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X}
\toprule
\textbf{Source} & \textbf{SS} & \textbf{ddof1} & \textbf{ddof2} & \textbf{F} & \textbf{p-value} & \textbf{eps} \\
\midrule
Search Agent & 2.34 & 1 & 20 & 6.73 & \textbf{.017} & 1.00 \\

Search Task & 0.24 & 2 & 40 & 0.63 & .48 & .68 \\

Search Agent \textasteriskcentered{} Search Task & 0.06 & 2 & 40 & 0.20 & .78 & .83 \\
\bottomrule
\end{tabularx}
\caption{Two-way repeated measures ANOVA results. SS (Sum of Squares): represents the variability in the dependent variable "Trust in Health Information". F (F-statistic): to determine whether the variability between group means is larger than the variability within the groups, higher F-values usually suggest the groups are different. P-value: represents the significance of the F-statistic. eps (Epsilon): Sphericity correction factor.}
% \vspace{-6mm}
\label{table:anova}
\end{table}
